Planning from Point Clouds over Continuous Actions for Multi-object Rearrangement

Long-horizon planning for robot manipulation is a challenging problem that requires reasoning about the effects of a sequence of actions on a physical 3D scene. While traditional task planning methods are shown to be effective for long-horizon manipulation, they require discretizing the continuous state and action space into symbolic descriptions of objects, object relationships, and actions. Instead, we propose a hybrid learning-and-planning approach that leverages learned models as domain-specific priors to guide search in high-dimensional continuous action spaces. We introduce SPOT: Search over Point cloud Object Transformations, which plans by searching for a sequence of transformations from an initial scene point cloud to a goal-satisfying point cloud. SPOT samples candidate actions from learned suggesters that operate on partially observed point clouds, eliminating the need to discretize actions or object relationships. We evaluate SPOT on multi-object rearrangement tasks, reporting task planning success and task execution success in both simulation and real-world environments. Our experiments show that SPOT generates successful plans and outperforms a policy-learning approach. We also perform ablations that highlight the importance of search-based planning.

==> tables/task_complexity_table.tex <==
\begin{wrapfigure}{r}{0.62\textwidth}
\vspace{-25pt}
\begin{minipage}{0.62\textwidth}
    \centering
    \renewcommand{\arraystretch}{1.2}
    \scriptsize
    \begin{tabular}{|r|c|c|c|c|}
        % \hline
        % \multicolumn{5}{|c|}{\textbf{Metrics as a function of task complexity}} \\
        \hline
         & \textbf{1 step} & \textbf{2 steps} & \textbf{3 steps} & \textbf{4 steps} \\
        \hline
        \textbf{Total search time (s)} & $1$ & $11$ & $32$ & $49$ \\
        \hline
        \textbf{Generated nodes} & $33$ & $391$ & $1123$ & $1711$ \\
        \hline
        \textbf{Expanded nodes} & $2$ & $20$ & $57$ & $86$ \\
        \hline
    \end{tabular}
    % \begin{tabular}{|r|c|c|c|c|}
    %     \hline
    %     \multicolumn{5}{|c|}{\textbf{Metrics as a function of task complexity}} \\
    %     \hline
    %      & \textbf{1 step} & \textbf{2 steps} & \textbf{3 steps} & \textbf{4 steps} \\
    %     \hline
    %     \textbf{Total search time (s)} & $14$ & $34$ & $27$ & $19$ \\
    %     \hline
    %     \textbf{Generated nodes} & $467$ & $1179$ & $978$ & $657$ \\
    %     \hline
    %     \textbf{Expanded nodes} & $24$ & $59$ & $49$ & $33$ \\
    %     \hline
    % \end{tabular}
    \vspace{-5pt}
    \captionof{table}{Metrics as a function of task complexity in the block stacking environment. Figures are averages. Search time is in seconds.}
    \label{tab:metrics}
\end{minipage}
\vspace{-15pt}
\end{wrapfigure}
